Faster Exact and Approximate Algorithms for $k$-Cut

In the $k$-cut problem, we are given an edge-weighted graph $G$ and an integer $k$, and have to remove a set of edges with minimum total weight so that $G$ has at least $k$ connected components. The current best algorithms are an $O(n^{(2-o(1))k})$ randomized algorithm due to Karger and Stein, and an $\smash{\tilde{O}}(n^{2k})$ deterministic algorithm due to Thorup. Moreover, several $2$-approximation algorithms are known for the problem (due to Saran and Vazirani, Naor and Rabani, and Ravi and Sinha). It has remained an open problem to (a) improve the runtime of exact algorithms, and (b) to get better approximation algorithms. In this paper we show an $O(k^{O(k)} \, n^{(2\omega/3 + o(1))k})$-time algorithm for $k$-cut. Moreover, we show an $(1+\epsilon)$-approximation algorithm that runs in time $O((k/\epsilon)^{O(k)} \,n^{k + O(1)})$, and a $1.81$-approximation in fixed-parameter time $O(2^{O(k^2)}\,\text{poly}(n))$.

==> approx-algo.tex <==

% \section{The DP algorithm}

% Our algorithm computes an approximation to $DP^*(v,s,R)$ for each $v\in V(T)$, $s\in[k-1]$, and $R\s I_v$ in time $(k/\e)^{O(k)}\poly(n)$. We will call our algorithm states $DP(v,s,R)$, in order to differentiate it with the ``ideal'' states $DP^*(v,s,R)$. Our main goal is to show that $DP(v,s,R)\approx DP(v,s,R')$ up to a small additive factor.

% \subsection{Partial vertex cover}\label{sec:pvc}
% The computation of each $DP(v,s,R)$ involves multiple calls to a problem well-studied in the FPT setting, known as partial vertex cover. We define a node-weighted version below.

% \begin{definition}[(Node-Weighted) Partial $k$-Vertex Cover]
% Given a graph $G$ with node weights $\varphi:V\to[0,\infty)$ and edge weights $\psi:E\to[0,\infty)$, the \emph{node-weighted partial $k$-vertex cover} problem is to find a set $S\s V$ of exactly $k$ nodes that minimizes $\varphi(S)+\psi(\bigcup_{v\in S}E[\{v\},V-\{v\}])$.
% \end{definition}

% The following theorem essentially follows from~\cite{gupta2018fpt}, with an improved running time from a more efficient coloring procedure and a separate, trivial case when $\el=1$. 
% \begin{theorem}
% There is an $(1+\delta)$-approximation algorithm for node-weighted partial $\el$-vertex cover that runs in time $(k/\delta)^{O(k)}\poly(n)$. In addition, if $\el=1$, then the algorithm is optimal.
% \end{theorem}
% \begin{proof}
% We follow the same strategy as Theorem 5.1 in~\cite{gupta2018fpt}, except with slightly different coloring probabilities. In their Lemma 5.2, instead of coloring each node red and blue with probability $\frac12$ each, we color them red with probability $1/\tau$ and blue with probability $(1-1/\tau)$, for $\tau:=\poly(k/\delta)$ as defined there. This way, following their definition, the probability that all the nodes in $S^*$ are colored red, and all the nodes in $N(S^*)\setminus S$ are colored blue is $(1/\tau)^k(1-1/\tau)^\tau = (\delta/k)^{O(k)}$. We thus repeat this step $(k/\delta)^{O(k)}\log n$ times, giving the desired running time.

% Finally, the case $\el=1$ can be trivially solved optimally, since the solution is simply the minimum weight node.
% \end{proof}

% Recall that, ideally, we want 
% \[
% DP^*(v,s,R) := \min_{\el^\dag,v_i^\dag,s_i^\dag,R_i^\dag} \lb \sum_{i=1}^\el DP^*(v_i^\dag,s_i^\dag,R_i^\dag) - \sum_{i=1}^\el\sum_{j=i+1}^\el w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)]) \rb,
% \]
% over all choices of $\el^\dag\in[s]$, distinct children $v_1^\dag,\lds,v_{\el^\dag}^\dag$ of $v$, positive integers $s_1^\dag,\lds,s_{\el^\dag}^\dag$ whose sum is $s$, and representatives $R_1^\dag,\lds,R_{\el^\dag}^\dag$ of $v_i^\dag,\lds,v_{\el^\dag}^\dag$ such that $R_i^\dag\s T_{v_i^\dag}$ and $T_{R_i^\dag} \cap I_v = R\cap T_{v_i^\dag}$ for each $i\in[\el^\dag]$. Of course, iterating over all possibilities may take $n^{\Om(k)}$ time, which is where we obtain the speedup via partial vertex cover.

% \paragraph{Setting up the instance.}
% The instance for computing $DP(v,s,R)$ is as follows. First, there is a guessing step, which is repeated multiple times. Let $\el$ be a uniformly random value in $[s]$, and for each child $u$ of $v$, let $s'(u)$ be a uniformly random value in $[s]$ and $R'(u)$ be chosen uniformly among those satisfying $R'(u)\s T_u$ and $T_{R'(u)}\cap I_v = R\cap T_u$. We say that our guessing procedure succeeds if $\el=\el^\dag$ and for each $v_i^\dag$, we have $s'(v_i^\dag)=s_i^\dag$ and $R'(v_i^\dag)=R_i^\dag$; we make no assumption on the children not in $\{v_1^\dag,\lds,v_{\el^\dag}^\dag\}$. Clearly, we succeed with probability at least
% \[
% \f1s \cd \lp \f1s \rp^\el \cd \lp \f1{2^{|T_{v_i^\dag}|}}\rp^\el = 2^{-\poly(k/\e)} .
% \]
% We will later repeat the procedure $2^{\poly(k/\e)}\log n$ times so that w.h.p., we succeed at least once. For a given procedure,  since there are two cases depending on whether $v\in R$, we split into two cases.

% \paragraph{Case 1: $v\notin R$.} 
% We construct the auxiliary graph $H$ on which to compute partial vertex cover. Let the children of $v$ be numbered $u_1,\lds,u_t$. For each child $u_i$, add a node of weight
% \[\varphi(u_i):=DP(u_i,s'(u_i),R'(u_i)) - \sum_{j=1}^t w(E[\sigma_v\inv(R'(u_i)),\sigma_v\inv(R'(u_j))])+M.\]
% Note that
% \[ \bigcup_{j=1}^t E[\sigma_v\inv(R'(u_i)),\sigma_v\inv(R'(u_j))] \s E[T_{u_i}, V-T_{u_i}] ,\]
% so
% \[ w(E[\sigma_v\inv(R'(u_i)),\sigma_v\inv(R'(u_j))]) \le w(E[T_{u_i}, V-T_{u_i}])\le M,\]
% and the node weight is always nonnegative.

% For each pair $u_i,u_j$, $1\le i<j\le t$, we add an edge $(u_i,u_j)$ in $H$ of weight
% \[ \psi(u_i,u_j):= w(E[\sigma_v\inv(R'(u_i)),\sigma_v\inv(R'(u_j))]) .\]

% If the (exact) optimal solution to \pvc is $S$, then that solution has value
% \begin{gather}
% \varphi(S)+\psi(\bigcup_{v\in S}E[\{v\},V-\{v\}])
% = \sum_{u\in S} DP(u,s'(u),R'(u)) + \el M 
%  - \sum_{\{u,u'\}\s S}w(E[\sigma_v\inv(R'(u)),\sigma_v\inv(R'(u'))]), \label{eq:PVCValue}
% \end{gather}
% since that all edges $(u_i,u_j)$ such that $u_i\in S$, $u_j\notin S$ get their weight canceled by the corresponding term in the negative summation of $\varphi(u_i)$. Observe that, aside from the additive $\el M$ and $DP^*$ being replaced by $DP$, the solution value is exactly the expression in the minimum from (\ref{eq:DPStarDef}) with values $\el$ and $u,s'(u),R'(u)$ for $u\in S$. Thus, if the guessing is successful, then the optimal value of \pvc is at most
% \begin{gather}
% DP(v_i^\dag,s_i^\dag,R_i^\dag) - \sum_{i=1}^\el\sum_{j=i+1}^\el w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)]) + \el M . \label{eq:PVCBound}
% \end{gather}
%  We now run $(1+\delta)$-approximate partial $\el$-vertex cover on $H$, for some $\delta:=\poly(\e/k)$, whose exact value is determined later. Because of this approximation, we suffer a small loss.

% The algorithm repeats the guessing and partial vertex cover computation $2^{\poly(k/\e)}\log n$ times. On each iteration, the algorithm writes down the value of the \pvc minus $\el M$, called the \textit{score} of that iteration. Finally, the algorithm sets $DP^*(v,s,R)$ as the value of the best score found. 

% \paragraph{Case 2: $v\in R$.} 
% Again, the nodes of $H$ consist of the children of $v$, numbered $u_1,\lds,u_t$. For each child $u_i$, 
% \begin{align*}
% \varphi(u_i):=DP(u_i,s'(u_i),R'(u_i)) &- w(E[\sigma_v\inv(R_i),V-T_v]) \\
%  & - \sum_{j=1}^t w(E[\sigma_v\inv(R'(u_i)),\sigma_v\inv(R'(u_j))])+2M,
% \end{align*}
% that is, the value in Case 1 with $- w(E[\sigma_v\inv(R_i),V-T_v])+M$ added on; again, we can show that the node weights are nonnegative. The edge weights $\psi(u_i,u_j)$ of $H$ are the same as in Case 1. Similarly, the algorithm repeats the procedure $2^{\poly(k/\e)}\log n$ times and on each iteration, writes down the value of the \pvc plus $\cut(\{v\})-2\el M$.

% The next lemma argues that in both cases, w.h.p., $DP(v,s,R)\approx DP^*(v,s,R)$.

% \begin{lemma}\label{lem:ActualDPApprox}
% W.h.p., for each vertex $v\in V(T)$, integer $s\in[k-1]$, and downward-closed subset $R\s I_v$, 
% \[
% DP^*(v,s,R) \le DP(v,s,R) \le DP^*(v,s,R)+(8s-4)\delta kM.
% \]
% \end{lemma}

% \begin{proof}
% We apply induction from the leaves of the tree to the root. We only prove the case $v\notin R$, since the other case is almost identical.

% The first inequality essentially follows by induction and (\ref{eq:PVCValue}). 
% For the second inequality, we split into the cases $\el^\dag=1$ and $\el^\dag\ge2$.

% If $\el^\dag=1$, then the single $DP(v_1^\dag,s_1^\dag,R_1^\dag)$ term introduces additive error $\le (8s-4)\delta kM$ by induction, and the \pvc algorithm outputs the optimal solution, so by (\ref{eq:PVCBound}), the score of a successful iteration is at most $DP^*(v,s,R)+(8s-4)\delta kM$. Since the algorithm takes the best score over all iterations, the second inequality holds.

% If $\el^\dag \ge2$, then by (\ref{eq:PVCBound}), the score of a successful iteration is at most
% \[ (1+\delta)\lp \sum_{i=1}^{\el^\dag} DP(v_i^\dag,s_i^\dag,R_i^\dag) - \sum_{i=1}^{\el^\dag}\sum_{j=i+1}^{\el^\dag} w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)]) + \el M \rp - \el M.\]
% We may assume that $DP(v_i^\dag,s_i^\dag,R_i^\dag)\le M$, since anything larger will not result in a solution that beats $M$, the value of the $2$-approximation algorithm. Therefore, the score is upper bounded by
% \[
% \lp \sum_{i=1}^{\el^\dag} DP(v_i^\dag,s_i^\dag,R_i^\dag) - \sum_{i=1}^{\el^\dag}\sum_{j=i+1}^{\el^\dag} w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)]) \rp
% + \delta \el M + (1+\delta) \el M  - \el M.
% \]
% By induction, \[DP(v_i^\dag,s_i^\dag,R_i^\dag) \le DP^*(v_i^\dag,s_i^\dag,R_i^\dag) - (8s_i^\dag-4)\delta kM.\]
% Thus,
% \begin{align*}
% DP(v,s,R) 
% &\le  \sum_{i=1}^{\el^\dag} DP(v_i^\dag,s_i^\dag,R_i^\dag) - \sum_{i=1}^{\el^\dag}\sum_{j=i+1}^{\el^\dag} w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)])  + 2\delta \el M \\
%  &\le  \sum_{i=1}^{\el^\dag} \lp DP^*(v_i^\dag,s_i^\dag,R_i^\dag) - (8s_i^\dag-4)\delta kM \rp - \sum_{i=1}^{\el^\dag}\sum_{j=i+1}^{\el^\dag} w(E[\sigma_v\inv(R_i^\dag), \sigma_v\inv(R_j^\dag)])  + 2\delta k M \\
% &= DP^*(v,s,R) - \sum_{i=1}^{\el^\dag} (8s_i^\dag-4)\delta kM + 2\delta k M \\
% &= DP^*(v,s,R) + (8s+ 2-4\el )\delta kM.
% \end{align*}
% Since $\el\ge2$, we have $8s+ 2-4\el \le 8s-4$, proving $DP(v,s,R) \le DP^*(v,s,R)+(8s-4)\delta kM$.
% \end{proof}

% \paragraph{Parameters.}
% There are two free parameters, $W=\poly(\e/k)M$ from \S\ref{sec:ImportantAndReps} and $\delta=\poly(\e/k)$ from \S\ref{sec:pvc}. By Lemma~\ref{lem:DPStarApprox} and Lemma~\ref{lem:ActualDPApprox},
% \begin{align*}
% DP(v,s,R) &\le DP^*(v,s,R)+(8s-4)\delta kM \\
% &\le \DQ(v,s,R) + (8s-4) \delta kM + (8s-4)k^2W \\
% &\le \DQ(v,s,R) + 8\delta k^2 M + 8k^3 W.
% \end{align*}
% Thus, setting $W:=\e/(32k^3)M$ and $\delta:= \e/(32k^2)$ gives
% \[ DP(v,s,R) \le \DQ(v,s,R) + (\e/2)M \]
% for all $v\in V(T)$, $s\in[k-1]$, $R\s T_v$. In particular, for the value $R^*\s T_{v_r}$ such that 
% \[\DQ(v_r,k-1,R^*)=w(OPT),\]
% we have
% \begin{align*}
%  DP(v_r,k-1,R^*) &\le \DQ(v_r,k-1,R^*)+(\e/2)M \\
% &\le  \DQ(v_r,k-1,R^*)+ \e\cd w(OPT) \\
% &=(1+\e)w(OPT),
% \end{align*}
% where we have used that $w(OPT) \ge M/2$, since $M$ is the value of a $2$-approximation algorithm. This concludes the $(1+\e)$-approximation algorithm, which runs in time $2^{\poly(k/\e)}\poly(n)$.


